Fast Approximate Vector Joins via Offline-Online Co-Design

Vector joins - finding all vector pairs between a set of query and data vectors whose distances are below a given threshold - are fundamental to modern vector and vector-relational database systems that power multimodal retrieval and semantic analytics. Existing state-of-the-art approach exploits work sharing among similar queries but still suffers from redundant index traversals and excessive distance computations. We propose a unified framework for efficient approximate vector joins that (1) introduces soft work sharing to reuse traversal results beyond the join results of previous queries, (2) builds a merged index over both query and data vectors to further speedup graph explorations, (3) improves robustness for out-of-distribution queries through an adaptive hybrid search strategy, and (4) further optimizes all these as offloading only the necessary online overhead to offline while minimizing maintenance cost. Experiments on eight datasets demonstrate substantial improvements in efficiency-recall trade-off over the state of the art.

==> 00.author_feedback_v2.tex <==
% ============================================================
%  AUTHOR FEEDBACK / RESPONSE  --  SIGMOD 2027, Paper 521
%  Rendered BEFORE the paper title (see \input in main.tex).
%  Anonymous: contains no author names or affiliations.
%  Target length: <= 2 pages.
%  Convention: \revised{}{...} = text written/updated by us this round (blue).
%             \torevise{note}{...} = a number/figure still to be filled (red).
% ============================================================
\begingroup
% Switch to two-column mode (same as the paper) with NO title banner.
\twocolumn[{\vspace*{-2\baselineskip}}]
%\small

% ===================================================================
% ALTERNATIVE OPENING (Option B) -- compare with the paragraph above.
% Keep ONLY ONE of the two for the final version.
% ===================================================================
%Forecast (top paragraph)

%No feeling - only facts / not written in the paper / we will write ...

%Go through reviews, top signal reviewers don't like the paper -- relevance / novelty / performance -- one sentence for each, from the paper (no number, capital, ...), pointer where in the current paper ...

%Make their effort minimum ... mention exact pointer ... "..." in Section X.

%BS -- scrutinize, divide sentences (likely to make reviewer accept the paper (green color) / not likely to have influence on the reviewers opinion (red color)) -- in this first paragraph 

%Texts should be shorter

%Answer with bullets - reviewer point in short / action (exp, place, ...) / time to do 
%- Reviewer point + 

We thank the reviewers for their insightful reviews{, and are encouraged that they find the idea \emph{elegant} (R2.S1) and \emph{well-motivated} (R1.S2), supported by \emph{comprehensive experiments} (R3.S3) with \emph{significant improvements at small radius} (R2.S2)}. %\revised{}{Several concerns stem from points we under-communicated in the submission, which we clarify below and will make explicit. As one highlight, a new experiment shows our adaptive hybrid search (\MIA) attains \emph{higher} recall than a dedicated state-of-the-art OOD index (CDMG+) while being \emph{faster} (Figure~\ref{fig:feedback}(c), G2(3)).}
We address general concerns (GX) and then respond to individual reviews.

% ===== PREVIOUS VERSION of G1 (before conceptual-reframe rewrite) =====
%\noindent\textbf{G1: Novelty.} We are the first to support fast threshold-based
%vector join with soft cross-query work sharing, encoder-centric
%merged indexing, and robust accuracy with OOD-aware adaptive
%hybrid search in one unified framework (Section 2), that captures existing state of the art [44], enables modular design, fair comparison, and clean ablations across a well-defined design
%space (Section 1), under a principle: shift as much join
%effort as possible to offline index construction, and handle only
%what cannot be anticipated offline at query time (Section 1).
%Simplicity is our deliberate design intent to be index-agnostic (Section 1), supported by experiments (Section 5.7), allowing us to satisfy all criteria in Table 1, \mbox{which was unattainable in related work (Section 2).}
%\revised{}{We see this simplicity as a strength, not a limitation: simple ideas that deliver large gains and generalize across indexes are, we believe, worth sharing with the community before developing yet another dedicated index. Strikingly, this even \emph{outperforms} a dedicated SOTA OOD index: our \MIA\ attains \emph{higher} recall and \emph{lower} latency than \INLJ\ over CDMG+ index (https://dl.acm.org/doi/10.1145/3786643, Figure~\ref{fig:feedback}(c), R1.O2). We will emphasize our novelty in Section 1 and add this experiment 5.}
% ===== END PREVIOUS VERSION =====
\noindent\textbf{G1: Novelty {(R2, R3: ``no novelty''; R2.O5: the techniques are individually simple)}.}
{We show} the bottleneck in vector join is \emph{a misalignment between the data's natural embedding geometry and the traditional table-centric index organization} (Section 1): since both sets come from the same encoder and already inhabit a shared embedding space, separate query/data indexes force the online phase to rediscover cross-set geometry for every join. Our key idea tackles this (Section 4.3): an \emph{encoder-centric merged index} encodes cross-set geometry offline and, via the relative-neighborhood-graph property, reduces initial in-range discovery to a \emph{threshold-agnostic, constant-time} neighborhood lookup (Section 4.3, Appendix C)---a hash-join-like design point for vectors (Table 2).
Around this we define one unified framework that captures the state of the art [44] as a special case, enabling modular design, fair comparison, and clean ablations (Section 1, 2), and stays index-agnostic (validated on NSG/HNSW, Section 5.7), satisfying all criteria in Table 1 \emph{for the first time}.
We see this simplicity as a strength, not a limitation: simple ideas that deliver large gains and generalize across indexes are, we believe, worth sharing with the community before developing yet another complicated, dedicated index. Strikingly, this even \emph{outperforms} a dedicated SOTA OOD index: our \MIA\ attains \emph{higher} recall and \emph{lower} latency than \INLJ\ over the open-source CDMG+ index (https://dl.acm.org/doi/10.1145/3786643, Figure~\ref{fig:feedback}(c), R1.O2). We will emphasize this novelty framing in Section 1 and add the CDMG+ experiment in Section 5.

%complicated, not work for in-distribution/mixed setup, ...

%\noindent\textbf{G1: Novelty.} \revised{}{Our novelty is conceptual, not a mere combination of techniques. We observe that shared-encoder query and data vectors already inhabit one geometric space, so the prevailing table-centric abstraction---separate query/data indexes---is misaligned with the data (Section 1, 2). Recasting it as an \emph{encoder-centric merged index}, we show via the relative-neighborhood-graph property that initial in-range discovery reduces to a \emph{threshold-agnostic, constant-time} neighborhood lookup, moving the dominant online cost offline (Section 4.3, Appendix C). Around this we define a unified offline--online design space that captures the state of the art [44] as a single configuration and enables clean, fair ablations (Section 1)---a combination unattainable in prior work (Table 1, Section 2). The resulting simplicity is a deliberate, index-agnostic choice (validated on NSG and HNSW, Section 5.7), not a lack of depth.}

% ===== PREVIOUS VERSION of G2(1) (reframed: small vs. large join size = two use cases) =====
%\noindent\textbf{G2: Performance.} \textbf{(1) Under large thresholds.} The main goal of work sharing and merged indexing has been to reduce the traversal effort in the greedy search (Section 5.2.3). For large thresholds, BFS (or hybrid search) equally becomes the bottleneck across all methods (Figure 10, Appendix E) that results in convergence/overlapping lines in Figure 8. The goal here is to find \emph{all} join results, and that there are too many results for large thresholds equally for all methods (up to more than $10^4$ per query, Figure \ref{fig:feedback}(a)). We chose a wide range for completeness, not only showing favorable cases. Still, large thresholds with large join sizes are less likely to be used in practice, similar to using small $k$ values (e.g., 5, 10, or 100) in typical top-$k$ ANN searches [32, 33], so we mainly focus on small threshold (Section 5.1.1). \cite{SimJoin} uses thresholds giving $\leq$10 results per query, which would have shown our benefits only, e.g., Figure \ref{fig:feedback}(b). We will make these clearer in the motivation of all techniques in Section 4 and experiments including the threshold design, emphasizing the results on small thresholds as in \cite{SimJoin} in Section 5.
% ===== END PREVIOUS VERSION =====
\noindent\textbf{G2: Performance.} \textbf{{(1) At large thresholds INLJ looks competitive and the lines in Figure 8 overlap (R1.O1).}}
Small and large thresholds are two genuinely different use cases. The dominant one is \emph{small} thresholds with small join sizes, the analogue of small $k$ in top-$k$ search [32, 33] (Section 5.1.1); \cite{SimJoin} likewise tunes thresholds to $\leq$10 results per query. There, work sharing and merged indexing target the greedy-search overhead---the main bottleneck under small thresholds (Section 5.2.3, Figure 10)---and our methods win decisively (Figure~\ref{fig:feedback}(b)).
\emph{Large} thresholds are a distinct, under-explored regime: there BFS (or hybrid search) dominates \emph{every} method, which must enumerate all (up to $>10^4$) results per query (Figure~\ref{fig:feedback}(a), Figure 10, Appendix E), so the lines converge in Figure 8. This degradation is universal---\cite{DiskJoin} also reports diminishing gains at large join sizes, and very recent work targets large-$k$ search specifically (arXiv:2604.01960)---and we do not claim to solve it. We report this unfavorable regime for a \emph{fair, complete} comparison, not only best cases; we will make this distinction explicit in Sections 2 and 5.

\noindent \textbf{{(2) \MIA and \MI look similar, and \MIA is sometimes slower than \MI, e.g., on \ImageNet (R1.O1, R3.O3).}} \MIA \emph{adaptively} enables OOD-aware hybrid search only for OOD queries (\ImageNet, \COCO, \LAION; Section 5.1.1), raising their recall while avoiding extra exploration on non-OOD queries, where it falls back to BFS and matches \MI's latency (Sections 1, 4.4, 5.2.1). We will make this explicit in Sections 1, 4.4 and 5.

\noindent \textbf{{(3) Gains from \MIA's adaptive hybrid search and soft work sharing (SWS) look marginal (R3.O3).}}
% ===== PREVIOUS VERSION (softened: lead with evidence, drop "respectfully disagree") =====
%\revised{}{The merged index is indeed our primary efficiency contribution, but we respectfully disagree that the gains from the other two are marginal.}
% ===== END PREVIOUS VERSION =====
The merged index is indeed our primary efficiency contribution; the other two, however, are far from marginal in the regimes they target.
%\MIA intentionally falls back to \MI for non-OOD cases. 
For OOD cases, all BFS-based methods lose recall, which is exactly the gap \MIA\ closes, improving recall by $\sim$43\% (Section~5.2.1).
Our \MIA\ even outperforms a dedicated SOTA OOD index, CDMG+, in both recall and speed (G1, Figure \ref{fig:feedback}(c)).
\SWS\ lowers latency by $\sim$3$\times$ over \HWS, and \HWS\
itself (\SimJoin \cite{SimJoin}) improves on the no-work-sharing \INLJ\ by $\sim$1.6$\times$ (Section~5.2.1).
The above CDMG+ paper shows $\sim$3.6$\times$ speedup compared to its baseline, similar gains to what \SWS gives. %Hence, $\sim$3$\times$ of SWS is not marginal, supported by those papers.
%This \HWS, hard work sharing, is the main idea in \SimJoin \cite{SimJoin}.
%In its paper, their efficiency gain is $\sim$3.6$\times$ 
%A SOTA OOD index named CDMG+ () also shows $\sim$3.6$\times$ speedup over its baseline.
%Therefore, $\sim$3$\times$ is not marginal in the literature.
%To our knowledge this 1.6\times is the first isolated
%measurement of hard work sharing: \SimJoin~[44] never reports its method with
%work sharing disabled, comparing only against a different system (VBASE), over
%which it reports up to about nineteen times; on the same footing, our merged
%index improves over hard work sharing by up to 44.1 times (Section~5.2.1). 
The per-query analysis in Section~5.3.1 confirms the benefit of
\SWS\ over \HWS\ is substantial. On recall, \SWS\ matches \HWS\ on most datasets
and even exceeds it on \GIST\ and \Glove; the small differences are index-structure
artifacts (Figure~12), not a weakness of soft sharing.
%\MIA is \emph{adaptive}, equals \MI for ID queries and only differs on OOD cases (\ImageNet, \COCO, \LAION) by enabling our hybrid search from the merged-index signal (Section 4.4).
%For OOD datasets all
%For OOD, all BFS-based methods lose recall, which is exactly the gap \MIA\
%closes, improving recall by up to 43\% (Section~5.2.1).
%The response to R1.O2 shows that \MIA has even higher recall than using the SOTA CDMG+ index in R1.O2.
We will clarify these and add CDMG+ experiment in Section 5 to strengthen our paper. 
%Please refer to R1.O3/O1 about why all methods largely converge at large thresholds.
%\MI\ and \MIA\ coincide on in-distribution data because the adaptive
%trigger spends extra out-range traversal only on hard OOD queries (Section~4.4),
%where \MIA\ improves recall by up to 43\% (Section~5.2.1).

%\MIA falls back to \MI for non-OOD cases.  


\noindent\textbf{G3: Relevance.} 
\iffalse
Threshold-based vector join over two same-encoder sets underlies cross-source product matching (Appendix A), deduplication, record linkage, recommendation, and fraud/security analytics (Section 1), run in batch over predefined sets like a relational join-key column (Section 3.1, Table 2) and predefined PK-FK relationship in schema design. Beyond listing domains, we will add a concrete example making two points explicit. 
(i) Threshold-agnostic reuse (Section 1 and 4.3).
In cross-source product matching, a marketplace joins its maintained catalog $Y$ against incoming seller batches $X$ encoded by the same model (Appendix A); the match threshold is not fixed but tuned per product category and to a target precision, and re-run as the catalog and seller uploads change. Since the merged index is built over the shared embedding space rather than for one threshold (Section 4.3), it is built once over X∪Y (and maintained incrementally as batches arrive, R2.O4) and reused across all these joins, amortizing the offline cost (R1.O3, R2.O1, R3.O1). (ii) An index over X∪Y, not per-set indexes. Here the repeated, dominant operation is the join (all matching catalog–seller pairs within the threshold), not single-set search; a single index over X∪Y turns initial in-range discovery into a constant-time neighborhood lookup (Section 4.3) and accelerates the join by ~44× (Section 5.2.1), whereas two per-set indexes are organized for single-set retrieval. A per-set catalog index is kept only when single-set product search is also frequent (R2.O3, Figure (d)). For multiple same-encoder sets (e.g., several seller catalogs), one union index with set labels serves all pairwise joins, avoiding N(N−1)/2 graphs (Section 4.3, R3.O2). We will add this example and promote Appendix A to the main text (Section 1).
\fi
% ===== PREVIOUS VERSION of G3 (before cross-source-product-matching rewrite) =====
%Threshold-based vector join over two sets from the same encoder is a primitive for AI-driven data management, underlying cross-source product matching, near-duplicate detection and deduplication, record linkage, recommendation, and fraud/security analytics (Section 1), with an end-to-end deployment scenario in Appendix A describing how our ideas fit.
%Such joins run in batch over predefined vector sets, analogous to a join-key column in relational joins (Section 3.1, Table 2) and predefined PK-FK relationship in schema design.
%Most importantly, all indexes are \emph{threshold-agnostic} (Section 1 and 4.3), so a pre-built index is reused across future thresholds and repeated batch joins rather than for a one-time query.
%We will surface these and the workload model in Section 1 and promote Appendix A to Section 4, emphasizing threshold-agnostic use cases (different thresholds are used for different downstream cases on the same data: a tight threshold to auto-accept high-confidence matching pairs, and a looser one to get a larger candidate set for a learned reranker or human review).
%
%While our merged index also supports single-set top-$k$ searches (R2.O3) and filters (Section 4.3), it is a \emph{join accelerator} for join-heavy or repeated-join workloads and complements per-set indexes for search-heavy ones (R2.O3, Figure \ref{fig:feedback}(d)). As it is index-agnostic, any existing index update mechanism can be used (Section 4.3). For multiple same-encoder sets, a single union index with set labels supports all pairwise joins, avoiding $N(N-1)/2$ graphs (Section 4.3). We will make these framing and index maintenance more explicit in Section 4.
% ===== END PREVIOUS VERSION =====
{\textbf{(R1.O3: in which applications is this used?; R2.O1, R3.O1: the offline index pays off only if the same two sets are joined repeatedly.)}
Threshold-based vector join is a fundamental primitive in AI-driven data management (Section 1): near-duplicate detection, record linkage, recommendation, fraud/security analytics, and cross-source product matching need \emph{all} pairs within a threshold $\theta$. Our merged index is widely applicable because it assumes only what these tasks already share---two sets from the \emph{same encoder} in one embedding space---and is \emph{threshold-agnostic} (built once, reused for any threshold; Section 1, 4.3) and \emph{index-agnostic} (any graph index; Section 1, 5.7); prior work instead maintains separate query/data indexes and rediscovers cross-set geometry per join (Section 1).
Repeated joins over a maintained pair are the norm, not the exception: in cross-source product matching (Section 1, Appendix A), a marketplace joins a maintained catalog $Y$ against incoming seller batches $X$ under the same encoder, exercising all three reuse axes: (i) the pair is re-joined on a schedule as data evolves, with the merged index maintained incrementally (R2.O4); (ii) it runs at many thresholds on the same data---a tight $\theta$ to auto-accept high-confidence pairs, a looser $\theta$ generates more candidates for a reranker or human review---reused without rebuilding (threshold-agnostic); and (iii) the same index also serves ordinary top-$k$ search on either catalog (R2.O3). Such joins run in batch over predefined sets, analogous to a join-key column (Section 3.1) and PK-FK relationship in schema design. For multiple same-encoder sets, one union index with set labels serves all pairwise joins, avoiding $N(N{-}1)/2$ graphs (R3.O2). The one-time offline index is thus amortized, not charged to a single query (R3.O1); 
%it \emph{complements} rather than replaces per-set indexes. 
it is a \emph{join accelerator} for join-heavy workloads and complements per-set indexes for search-heavy ones (R2.O3, Figure \ref{fig:feedback}(d)).
We will promote Appendix A to the main text and make this workload model explicit in Sections 1 and 4.}


\noindent \textbf{Plan:} Due to space, we appreciate any questions (misread/unresolved concerns, required experiments, applications). We will provide all details in the discussion. A major revision will take $\leq$2 weeks.

%and will give all details in the discussion; a major revision needs approx.\ 2 weeks.

\iffalse
We sincerely thank the reviewers for their comments, 
and we are encouraged that the idea is found \emph{elegant} (R2.S1), \emph{novel
and well-motivated} (R1.S2), and supported by \emph{comprehensive experiments}
with \emph{significant improvements at small radius} (R2.S2, R3.S3). After
studying the reviews carefully, we believe all concerns except R2.O3 can be resolved
without difficulty, and in fact that the submission already answers many of
them---in its text, footnotes, figures, and appendices---which we should have surfaced more
clearly. We sincerely apologize and commit to making them explicit, 
in particular applications in Section 1 / Appendix A (R1-3); 
all indexes are \emph{threshold-agnostic} so can be reused for any join threshold (R1.O3, R2.O1, R3.O1); the adaptivity of \MIA (R1.O1, R3.O3), which triggers hybrid
search only for queries predicted OOD from the
merged-index signal and otherwise falls back to BFS, coinciding with \MI\ on
in-distribution (ID) queries; and following the problem setup of \SimJoin\ \cite{SimJoin} (R2.O2).
%For R2.O3, by making the
%\emph{single-set-search-versus-join} trade-off explicit---so that a practitioner
%can choose between a search-heavy and a join-heavy deployment by weighing a
%dedicated per-set index against the merged index---will, we believe, strengthen
%the paper, and we develop this trade-off in our response below.
Due to space limitation, we would be grateful for taking any further questions, especially for misread/misanswered/unresolved concerns, further required experiments, and application scenarios. 
We are happy to provide all in the discussion phase than deferring to the revision.
% ===================================================================
% end ALTERNATIVE OPENING
% ===================================================================
\fi

\begin{figure*}[t]
\centering
\begin{minipage}[b]{0.22\textwidth}\centering
\includegraphics[width=\linewidth]{feedback_figure/joinsize_avg_per_query.png}\\[-7pt]
{\footnotesize (a)}
\end{minipage}\hfill
\begin{minipage}[b]{0.265\textwidth}\centering
\includegraphics[width=\linewidth]{feedback_figure/combined_results_sift_new_thresholds_median.png}\\[-7pt]
{\footnotesize (b)}
\end{minipage}\hfill
\begin{minipage}[b]{0.24\textwidth}\centering
\includegraphics[width=\linewidth]{feedback_figure/combined_results_nsg_inlhybrid_cdmg_v3_imagenet_median.png}\\[-7pt]
{\footnotesize (c)}
\end{minipage}\hfill
\begin{minipage}[b]{0.253\textwidth}\centering
\includegraphics[width=\linewidth]{feedback_figure/ratio_sweep_per_set.png}\\[-7pt]
{\footnotesize (d)}
\end{minipage}
\vspace*{-0.35cm}
\caption{
\textbf{(a)} Avg. join size $k$ per query vs.\ our thresholds used in Section 5; the band $k \leq 10$
is \SimJoin's~\cite{SimJoin} regime.
\textbf{(b)} Finer \SIFT\ thresholds calibrated to $k=1,\dots,10$:
\MI/\MIA\ stay about an order of magnitude faster than \INLJ/\HWS/\SWS\ at recall
$\approx$1.
\textbf{(c)} On the OOD dataset \ImageNet, \INLJ\ with forced hybrid search (no adaptivity allowed based on merged-index signal, Section 4.4) and
\INLJ\ over the state-of-the-art OOD graph index CDMG+ both improve recall but
remain below \MIA.
\textbf{(d)} Single-set top-$10$ search (ANNS) on {a per-set index over $Y$ vs.\ the merged index over $X\cup Y$} on
\SIFT\ (merged index fixed at $1$M vectors): recall matches while the merged-index latency decreases from $\sim$25$\times$ to $\sim$1.3$\times$ as {$|Y|/|X\cup Y|$} grows from 1\% to 45\%.}
\label{fig:feedback}
\vspace*{-0.5cm}
\end{figure*}

\vspace{0.1cm}
\textbf{Response to Reviewer 1}

\noindent\textbf{R1.O1.} %As noted, all methods converge at large thresholds. % due to the large number of results that BFS (or hybrid search) has to find.
{Please refer to G2(1).} We will emphasize the small-threshold area (Figure \ref{fig:feedback}(b)) and the convergence under large thresholds, and replot with more distinct colors/markers.
%%, and move large thresholds to the end.
%The convergence the reviewer observed at large thresholds is
%expected rather than a failure: there all methods become bottlenecked by the
%BFS expansion that traverses most in-range points (Figure~10, Appendix~E), so
%the join-level optimizations (\SWS, \HWS, \MI), which target the greedy-search
%overhead, can no longer separate the methods; large thresholds are rare in
%practice, the analogue of large $k$ in top-$k$ search. Notably, the
%state-of-the-art \SimJoin~[44] tunes its threshold so that each query returns
%only about one to ten matches, which corresponds to our two smallest thresholds
%(Figure~\ref{fig:feedback}(a)). To test this realistic regime directly, we
%re-ran on \SIFT\ with ten finer thresholds calibrated to an average join size of
%exactly $k=1,2,\dots,10$ (\SimJoin's coverage): \MI\ and \MIA\ stay about an
%order of magnitude faster than \INLJ, \HWS, and \SWS\ at recall $\approx$1.0
%throughout (Figure~\ref{fig:feedback}(c)), so our advantage is fully retained
%where joins are realistically run. 
For \NYTimes\ at $\theta_7$, \INLJ\ is faster
but at lower recall, and \MIA's recall decreases due to 
1) the low connectivity of the index (low ``mode'' in Table 4) over highly-skewed data and
2) large per-query join size (Figure \ref{fig:feedback}(a)).
{Finally, see G2(2) for why \MIA is slower but has higher recall than \MI on OOD datasets, e.g., \ImageNet.}
%\revised{}{Finally, on why \MIA\ and \MI\ look similar---\MIA\ equals \MI\ for ID queries and enables hybrid search only for OOD---see G2(2).}

%where it deliberately traverses a bounded number of out-range bridges
%(Algorithm~7) to repair the recall that BFS alone loses; this costs extra latency
%but stays below the separate-index methods in our small-threshold regime, because
%\MI\ already removes most greedy-search cost. In short, \MIA\ and \MI\ both
%improve over \INLJ, and on OOD data \MIA\ trades a little latency for the highest
%recall.

\noindent\textbf{R1.O2.} Typo: in our INLJ description (Section 5.2.1) the OOD recall drop (\COCO/\LAION) is not due to low node degree but due to disconnected in-range regions (Section 4.4), which we will correct.
All methods except \MIA use BFS expansion (Section 3.2.2, 4.1). In Figure \ref{fig:feedback}(c), INLJ+Hybrid replaces BFS with our OOD hybrid search, and INLJ (CDMG+) replaces the underlying NSG with CDMG+ (please refer to G1); we used CDMG+ since the requested NGFix paper isn't open-source, but will implement it if asked. \MIA stays much faster at small thresholds (then converges, G2(1)) with consistently higher recall (same for \COCO, \LAION). We will add these in Section 5.


\noindent\textbf{R1.O3.} 
%The thresholds in Table~5 are evenly spaced
%per dataset, identical across all baselines, and not tuned to favor us; they
%deliberately span from sparse to dense joins (Figure~7). 
%Please refer to our last two paragraphs in Section 5.1.1, %with "we mainly focus on small thresholds (e.g., $\theta_1$ to $\theta_3$) and show the results for larger thresholds for completeness." 
%which is the first reason for using the thresholds in Table 5; 
We designed thresholds to cover a wide range for completeness, including large thresholds where all methods converge and the realistic small thresholds where our gains are largest {(Section 5.1.1, G2(1)).} %so including the unfavorable large-threshold cases
%for completeness has less impact on realistic workloads.
\iffalse
Second, as there is no common benchmark for threshold-based vector joins, 
we wanted to reflect how actual users would input thresholds, e.g., in exploratory analysis.
We asked students to play with our prototype 
%only query/data size and avg. distance between vectors.
and observed a common pattern that they preferred trying evenly-spaced and round numbers (e.g., 50, 70, 90, and then converge to small thresholds for higher interactivity and join size sensitivity). So we chose evenly-spaced thresholds that cover small-to-large frequently tried numbers. We will add this info in Section 5.
\fi
For application, {please refer to G3.}
%we will promote the deployment scenario (Appendix~A) 
%to the main text, with \emph{threshold-agnostic} (Section 1, 4.3) examples added, i.e., same index reused across any threshold (please see R2.O1 below).
%report a short study of how users choose thresholds given only the vector sets
%\torevise{add study/numbers}{(we observed a consistent preference for round,
%evenly-spaced values)}.


%\section*{Reviewer 2}
\vspace{0.1cm}
\textbf{Response to Reviewer 2}

\noindent\textbf{R2.O1, R2.Q1.} Please refer to G3 {(use cases) and R3.O1 (the $10^3$\,s build is the standard ANN-index cost, amortized---not a one-time surcharge)}, alike \SimJoin \cite{SimJoin}.
%Both separate/merged
%indexes are \emph{threshold-agnostic}, built \emph{once} and reused across future thresholds, recurring joins over maintained tables (Appendix A), rather than for a one-time join query. %Such repeated joins over a shared embedding space are common in practice (applications in G3).
%supporting vector joins with any input threshold. 
%they encode proximity in the shared embedding space, not a particular threshold (Section~4.3), so a pre-built index
%reused for joins at any future threshold and even plain top-$k$ search for any $k$ on either set (R2.O3). 
%The two sets to be joined are known in advance \revised{}{(similar to PK-FK relationship in schema design), as with recurring joins over maintained tables (or materialized access paths) in analytical pipelines,} and our merged index is maintained over all vectors from the \emph{same embedding space} (Section 1, 4.3) also known in advance.
%As in filtering each table, we can apply filters on the right using the post-filtering approach in the literature, and naively on the left.
%Merged index can be used for plain top-$k$ search on either set (R2.O3).
%Section 4.3 discusses the benefit of merged index for left-side filters.
%We will make these explicit in Section 4 as well as the applications from G3.
%product matching scenario state threshold-agnostic reuse explicitly -- the merged index is built once over the shared embedding space and reused for joins at any future threshold, amortizing the one-time offline cost -- promote it to the main text, and emphasize other applications in Section 1 and 4.3.
%and promote the deployment scenario in Appendix A to the main text, with threshold-agnostic examples -- 

\iffalse
The strongest amortization is a \emph{fixed pair joined repeatedly}:
recurring record linkage between two maintained databases; benchmark-contamination
detection, which joins every new evaluation set against one training corpus
indexed once, under the same encoder, at a tunable cutoff; or cross-lingual
bitext mining, a margin/threshold join between two language collections in one
multilingual space, re-run across many language pairs. A second mode is a
\emph{stable reference with streaming queries}: in cross-source product matching
(Appendix~A) the catalog is indexed once and each small seller batch is
\emph{inserted incrementally} (the mechanism of R2.O4), not rebuilt. In all of
these the build is the standard ANN index one already maintains, incurred once
and shared; the merged organization adds at most 4.5\% in
size and 0.7\% in time over two separate indexes (Section~5.5; Theorem~1,
Appendix~B). The merged index also supports filters on either side by pre- or
post-filtering, and is the only one of the two that preserves left-side work
sharing under filters, since filtering the query set can disconnect the left-side
graph and its ordering (Section~4.3).
\fi

\noindent\textbf{R2.O2, R2.Q2.} \SimJoin \cite{SimJoin}'s left (query) index is
built \emph{fully} offline, exactly as ours; only the Minimum Spanning Tree (MST) is done online over that graph index to schedule left vectors for work sharing, and that time is negligible (Section~3.2.3, \cite{SimJoin}). 
%\HWS\ is our faithful reimplementation of \SimJoin\
%inside the unified framework, using the same offline query and data indexes and
%the same MST-based hard work sharing (Section~5.1.2). 
We reimplemented \SimJoin because the authors declined to share their code; our version reaches per-query join latency at small thresholds similar to \cite{SimJoin}'s (see footnote~1).
%and neither \XJoin\ nor \DiskJoin\ is open-sourced either
%(footnote~2). The comparison is therefore against \SimJoin, under matched
%offline-index assumptions.

\noindent\textbf{R2.O3.}
% ===== PREVIOUS VERSION of R2.O3 framing (this scope statement promoted to G3) =====
%We thank the reviewer for this; making the search-vs-join trade-off explicit strengthens the paper.
%{We will state the intended workload model explicitly: the merged index is \emph{not} meant to replace per-set indexes for every workload. It is primarily a \emph{join accelerator} for join-heavy or repeated-join workloads over a shared embedding space, and it \emph{complements} rather than replaces {per-set} indexes for searches.}
% ===== END PREVIOUS VERSION =====
We thank the reviewer; making the search-vs-join trade-off explicit strengthens the paper. The workload model and scope are stated in G3 (the merged index \emph{complements} rather than replaces per-set indexes); here we quantify the trade-off.
Since the merged index is larger, a single-set top-$k$ search on it traverses many out-set nodes before collecting enough in-set ones, so it is slower than on a per-set index.
\iffalse
Theoretically, the search complexity is $O(log N)$ for a $N$-node index, so the difference $O(log N) - O(log rN) = O(log 1/r)$ is bounded for the single-set-to-merged index size $r < 1$. In practice,
\fi
%\revised{}{We can theoretically prove that this additional overhead is bounded, and}
%in practice, 
On \SIFT\ (Figure~\ref{fig:feedback}(d)), single-set top-$10$ search on the merged index matches the {per-set} index's recall,
while its relative latency depends on the {ratio $r=|Y|/|X\cup Y|$}: $1.3\times, 2\times, 5\times$, and $10\times$ for $r = 0.45, 0.2, 0.06$, and $0.03$.
%on how large the searched set is
%relative to the union: about $1.3\times$ when the searched set is $\sim$45\% of
%the union, growing to roughly $25$--$30\times$ when it is only $\sim$1\%.
%the integer label-skip of our $N$-set extension (R3.O2) reduces this, and when the
%two sets coincide the merged index reduces exactly to one ordinary index.
This is a clean knob: for join-heavy workloads the modest single-set overhead is outweighed by the $\sim$44$\times$ join speedup; for search-heavy ones, one keeps a {per-set} index alongside (only for small $r$; maintenance cost $(1{+}r)\times$, at most $2\times$), optionally switching between them adaptively (future work). We will add this trade-off in experiments and the conclusion.

%which costs only
%about $1/\kappa$ extra \emph{storage} (the smaller set is $\kappa$ times smaller
%than the union). One can even maintain this adaptively---favoring separate
%indexes when joins are infrequent and the merged index when they are
%frequent---which we see as interesting future work. We will add this discussion
%and Figure~\ref{fig:feedback}(d).

\noindent\textbf{R2.O4.} {Since the merged index is index-agnostic (Section 1, 4.3; Table 1),
%any index maintenance mechanism is applicable (Section 4.3). over same-encoder vectors with set labels (Section 4.3), 
existing index maintenance mechanisms apply directly [32, 37], and thus maintenance optimization is orthogonal to our paper. 
A node update needs no left/right distinction, only its set label to be used for joins/searches. We will add a short maintenance subsection discussing incremental updates and periodic batch rebuilds.}
%and an update experiment available on request.

\noindent\textbf{R2.O5 (and novelty).} Please refer to G1.
%\revised{}{On novelty and the deliberate simplicity of our index-agnostic, generalizable design (capturing \SimJoin\ as a special case and satisfying all criteria in Table 1), see G1. We add that the response to R1.O2 (and G2(3)) shows \MIA\ is even faster and/or higher in recall than applying a dedicated SOTA OOD index per set.}

%Figure (c) shows that it's even faster, accurate than SOTA OOD dedicated index.
%And novelty is not in simplicity, but elegance, motivation, connection, insights, ... 

%\section*{Reviewer 3}

\vspace{0.1cm}
\textbf{Response to Reviewer 3}

% ===== PREVIOUS VERSION of R3.O1 (was a bare pointer; build-cost rebuttal added) =====
%\noindent\textbf{R3.O1.} Please refer to {G3}.
% ===== END PREVIOUS VERSION =====
\noindent\textbf{R3.O1.} Please refer to G3 for repeated-join use cases. On the $10^3$\,s build: this is the standard graph-ANN index-construction cost, not a join-specific surcharge---building our merged index costs essentially the same as the two ordinary per-set indexes one already maintains for search (up to $+4.5\%$ size, $+0.7\%$ time; Section 5.5, Figure 15). Moreover, the index is not built for a single join: it is reused across all future thresholds (threshold-agnostic, Section 4.3) and also serves ordinary top-$k$ search on either set (R2.O3, Figure~\ref{fig:feedback}(d)), so the one-time cost is amortized over many joins and searches, not charged to one query. We will make this explicit from Section 1. %: both separate and
%the merged indexes are built once and threshold-agnostic, reused for any future thresholds.
%\revised{}{The $10^3$-second build is the standard ANN index cost one already pays for ordinary search, incurred once and shared across all future joins and thresholds, not charged to a single one-time join.}
%We will make this explicit in Section 4.
%{top-$k$ searches, filters, and repeated batch joins, 
%but with a different search-vs-join trade-off (R2.O3).}
%\revised{}{The $10^3$-second build is the standard ANN index cost one already pays for ordinary search, incurred once and shared across all future joins, thresholds, filters, and repeated batches---not charged to a single one-time join.} We will make this explicit.
%The $10^3$-second cost is the standard ANN index build, shared rather than charged
%to each join, and the merged organization adds under 5\% over the indexes one
%already maintains (Section~5.5).

\noindent\textbf{R3.O2.} Merged index is encoder-centric: Section 4.3 builds a \emph{single} index over all same-encoder sets (we focus on the common case of two), {so we do \emph{not} need $N(N{-}1)/2$ pairwise graphs}.
%"If multiple vector sets are produced by the same encoder, they can be indexed
%jointly in a single structure; in this paper, we focus on the common
%case of two sets, $X$ and $Y$." 
%When the sets are produced by the same encoder (known in advance, R2.O1), we do not build $N(N{-}1)/2$ graphs but a \emph{single} index over all of them, 
So the index overhead is linear in the total number of vectors, and per-vector \emph{set labels} support joins across any pair of sets.
%---a join simply restricts traversal to the two relevant labels---so we do \emph{not} need $N(N{-}1)/2$ pairwise merged graphs; 
We will make this explicit in Section 4.
%We have preliminary results on more than two sets, but it 

%not quadratic in the number of sets; the join keys are
%known from the schema (R2.O1), so only the needed sets are indexed. The genuine
%difficulty the reviewer raises---that a third set can act as a
%\emph{disconnector} (lowering recall) or, if fully traversed, inflate latency---
%is real, and we have already designed and prototyped a set-aware extension:
%set-partitioned adjacency that skips foreign-set neighbors by an integer label
%check with no distance computation (the bottleneck); set-aware edge augmentation
%that keeps each set's induced subgraph navigable; triangle-inequality range
%pruning from stored edge lengths; and a bounded online bridging budget as an
%explicit recall--latency knob. On a synthetic study ($|Y|{=}1000$, with a
%disconnector set $Z$ drawn from the same mixture so it interleaves with $Y$;
%$C$~is distance computations per query):

\iffalse
{\color{blue}\footnotesize
\begin{center}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lccc@{}}
\toprule
$|Z|$ & strict $Y$-BFS & full traverse & \textbf{set-aware ext.} \\
\midrule
0      & R=0.98, C=86  & R=1.00, C=90  & \textbf{R=1.00, C=90} \\
1{,}000  & R=0.91, C=123 & R=1.00, C=156 & \textbf{R=1.00, C=137} \\
4{,}000  & R=0.69, C=163 & R=1.00, C=348 & \textbf{R=1.00, C=138} \\
10{,}000 & R=0.39, C=130 & R=1.00, C=701 & \textbf{R=1.00, C=135} \\
\bottomrule
\end{tabular}
\end{center}}

\revised{}{Strict same-set BFS collapses to 0.39 recall as $Z$ grows, while full
traversal keeps recall only at a cost linear in the data size; our extension
holds recall near 1.0 at roughly flat cost, about five times fewer distance
computations at the largest $|Z|$. We will develop this as the $N$-set extension
and validate it on real datasets \torevise{add real-data experiment and overlay
overhead}{[results to be added]}.}

\fi

\noindent\textbf{R3.O3.} {Please refer to G2(2) for why \MIA and \MI look similar on non-OOD datasets, and G2(3) for the non-marginal gains of \SWS and adaptive hybrid search.}
%\revised{}{We respectfully disagree that the gains are marginal. The \SWS/\HWS\ comparison ($\sim$3$\times$), the CDMG+ context ($\sim$3.6$\times$), the per-query analysis (Section 5.3.1), and the recall artifacts (Figure 12) are in G2(3); the adaptivity of \MIA---equal to \MI\ for ID queries and improving OOD recall by up to 43\% (Section 5.2.1)---is in G2(2); and why all methods converge at large thresholds is in G2(1). We will add all these to the experiments and related work.}
%\MI\ and \MIA\ coincide on in-distribution data because the adaptive
%trigger spends extra out-range traversal only on hard OOD queries (Section~4.4),
%where \MIA\ improves recall by up to 43\% (Section~5.2.1).

\noindent\textbf{R3.O4.} %We apologize for making this unclear. 
{Our framework does \emph{not} discard beam search: its greedy phase \emph{is} a standard beam (best-first) search, only it stops at the first in-range node rather than ranking top-$k$, then transitions to BFS (Section~4.1.2--4.1.3). We adopt this two-phase design because beam search alone cannot serve a threshold join (Section 4.4, Figure 5): it needs the result size $k$ in advance, but the in-range count is unknown and varies widely across queries and thresholds.}
%Our greedy-then-BFS search is thus the
%principled adaptation of beam search to thresholds, not an arbitrary replacement.
%The framework also captures \INLJ\ and \SimJoin\ as configurations (Figure~1), so
%\INLJ\ already serves as the per-query standard-ANNS baseline. 
For a direct comparison for single-set top-$k$ searches, please refer to R2.O3 and Figure~\ref{fig:feedback}(d).

\noindent\textbf{R3.Q1.} We explain this in Section~4.1.2 and~5.2.2:
the greedy search only needs to reach \emph{one} in-range point (not
top-$k$), so enlarging the queue does not change recall much. 
The post-greedy BFS has no queue-size limit; only \MIA's hybrid search limits queue size for out-range nodes, so a larger queue allows traversing more out-range nodes as bridges to discover more in-range regions, increasing recall at a higher latency (Figure~9). We will make these clearer.

\noindent\textbf{R3.M1 (minor).} We will replace Figure~15 with a table, showing merged index actually slightly reduces the overhead overall.
%of index size and build time (separate vs.\ merged), confirming the up-to 4.5\% and 0.7\% overhead (Section~5.5). 
%More precisely, the merged index's index size is equal or lower in 5 of 9 datasets, and build time is equal or lower in 8 of 9.
%\torevise{insert table}{[table]}.

\normalsize
\endgroup
\clearpage


